On counting associative submanifolds and Seiberg-Witten monopoles

Building on ideas from [DT98; DS11; Wal17; Hay17], we outline a proposal for constructing Floer homology groups associated with a G2-manifold. These groups are generated by associative submanifolds and solutions of the ADHM Seiberg-Witten equations. The construction is motivated by the analysis of various transitions which can change the number of associative submanifolds. We discuss the relation of our proposal to Pandharipande and Thomas' stable pair invariant of Calabi-Yau 3-folds.

==> ADHMSeibergWittenEquations.tex <==
\section{The ADHM Seiberg--Witten equations}
\label{Sec_ADHMSeibergWittenEquations}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "CountingAssociativesSeibergWitten"
%%% End:


==> CoupledFunctional.tex <==
\section{Coupled Chern--Simons--Dirac functionals}
\label{Sec_CoupledFunctional}

\subsection{Associative submanifolds and monopoles}

An immersion $\iota\in \Imm_\beta(P,Y)$ is associative if and only if it is a critical point of the functional $\fL$ introduced in \autoref{Sec_LFunctional}.
Likewise, a pair $(\Psi,A)\in \Gamma(W) \times \sA(\det W)$ is a solution of the Seiberg--Witten equation \eqref{Eq_ClassicalSeibergWitten} if and only if it is a critical point of the Chern--Simons--Dirac functional $\CSD$ introduced in \autoref{Sec_AssociativeMonopoleHomology}.
The coupled condition that $\iota$ is associative and $(\Psi,A)$ satisfies the Seiberg--Witten equation with respect to $\iota^*g$ is not equivalent to $(\iota,\Psi,A)$ being a critical point of any naturally defined functional.
However, it does appear as the decoupling limit of a family of critical point equations.

\begin{definition}
  Given a \defined{coupling constant} $\kappa > 0$,
  we define the \defined{$\fL$--Chern--Simons--Dirac functional} $\fL\CSD_\kappa\co \tImm_\beta(P,Y) \times \Gamma(W) \times \sA(\det W) \to \R$ by
  \begin{equation*}
    \fL\CSD_\kappa(\iota,[Q],\Psi,A)
    \coloneq
    \int_Q \psi
    + \kappa\(\frac12\int_P (A-A_0)\wedge F_A
    + \int_P \inner{\slD_{A,\iota^*g}\Psi}{\Psi} \vol_{\iota^*g}\).
  \end{equation*}
\end{definition}

\begin{prop}
  \label{Prop_LCSD}
  Given $\kappa >0$,
  $(\iota,[Q],\Psi,A)$ is a critical point of $\fL\CSD_{\kappa}$ if and only if the pair $(\Psi,A)$ satisfies the Seiberg--Witten equation on $P$ with respect to the Riemannian metric $\iota^*g$:
  \begin{equation}
    \label{Eq_IotaClassicalSeibergWitten}
    \begin{split}
      \slD_{A,\iota^*g} \Psi
      &=
      0 \qand \\
      \frac12 F_A
      &=
      \mu_{\iota^*g}(\Psi),
    \end{split}
  \end{equation}
  and for every positive orthonormal basis $(e_1,e_2,e_3)$ and $n \in N_x\iota$
  \begin{equation}
    \label{Eq_PsiAssociative}
    \inner{[\iota_*e_1,\iota_*e_2,\iota_*e_3]}{n}
    =
    \frac{\kappa}{2} \sum_{i=1}^3 \inner{\gamma(e_i)\nabla_{A,\rII_\iota(n)e_i}\Psi}{\Psi}.
  \end{equation}
  Here $\gamma$ denotes the Clifford multiplication and $\rII_\iota \in \Gamma(S^2T^*P\otimes N\iota) \subset \Gamma(N\iota^*\otimes \End(TP))$ the second fundamental form of the immersion $\iota$.
\end{prop}

\begin{remark}
  If $\kappa = 0$, then \eqref{Eq_PsiAssociative} is simply the condition that $\iota$ is associative.
\end{remark}

\begin{proof}[Proof of \autoref{Prop_LCSD}]
  Let $(\iota,[Q],\Psi,A) \in \tImm_\beta(P,Y) \times \Gamma(W) \times \sA(\det W)$.
  Denote by $H_\iota = \tr \rII_\iota \in \Gamma(N\iota)$ the mean curvature of $\iota$.
  We define the \defined{stress-energy tensor} $T_{\Psi,\iota^*g} \in \Gamma(S^2T^*P)$ of $\Psi$ with respect to $\iota^*g$ by
  \begin{equation*}
    T_{\Psi,\iota^*g}(v,w)
    \coloneq
    \inner{\gamma(v)\nabla_{A,w}\Psi+\gamma(w)\nabla_{A,v}\Psi}{\Psi}.
  \end{equation*}
  Using the variation formula for the Dirac operator, cf.~\citet[Thèorème 21]{Bourguignon1992} and \citet[Lemma 2.3]{Branding2016}, we obtain
  \begin{align*}
    &\rd_{(\iota,[Q],\Psi,A)}\fL\CSD_\kappa(n,\hat\psi,a) \\
    &\quad= 
      \int_P \iota^*i(n)\hat\psi
      - \frac{\kappa}{4} \int_P \inner{T_{\Psi,\iota^*g}}{\rII_\iota(n)}\, \vol_{\iota^*g}
      + \frac{\kappa}{2} \int_P \inner{H_\iota}{n} \inner{\slD_{A,\iota^*g}\Psi}{\Psi}\, \vol_{\iota^*g} \\
    &\qquad+
      \kappa\(
      \int_P a \wedge F_A + \inner{\bar\gamma(a)\Psi}{\Psi} + 2\inner{\slD_{A,\iota^*g}\Psi}{\psi} \).
  \end{align*}
  If $(\iota,[Q],\Psi,A)$ is a critical point of $\fL\CSD_\kappa$,
  then setting $n = 0$ and varying $\hat\psi$ and $a$ shows that $(\Psi,A)$ satisfies the Seiberg--Witten equation with respect to $\iota^*g$.
  In particular, $\slD_{A,\iota^*}\Psi=0$ and the third term vanishes.
  The resulting condition on $\iota$ is
  \begin{equation*}
    \inner{[\iota_*e_1,\iota_*e_2,\iota_*e_3]}{n}
    =
    \frac{\kappa}{2} \sum_{i=1}^3 \inner{\gamma(e_i)\nabla_{A,\rII_\iota(n)e_i}\Psi}{\Psi}.
    \qedhere
  \end{equation*}  
\end{proof}

Equation \eqref{Eq_PsiAssociative} has some similarities with Dirac-harmonic maps introduced by \citet{Chen2004a}.
It is an interesting question whether the more strongly coupled equations \eqref{Eq_PsiAssociative} and \eqref{Eq_IotaClassicalSeibergWitten} for $\kappa > 0$ instead $\kappa = 0$ might have a regularizing effect.
In particular, it would be interesting to understand what happens to the singularities encountered in \autoref{Sec_IntersectingAssociatives} and \autoref{Sec_AssociatviesWithT2Singularities}  when $\kappa$ is deformed from $\kappa = 0$ to $\kappa > 0$.


\subsection{Holomorphic curves and vortices}

Like associative submanifolds, holomorphic curves in a Calabi--Yau $3$--fold are critical points of a functional on the space of submanifolds.

\begin{definition}
  For a closed, oriented surface $\Sigma$,
  let $\Imm(\Sigma,Z)$ be the space of immersions from $\Sigma$ to $Z$.
  Define a complex $1$--form $\delta\fL^\C \in \Omega^1(\Imm(\Sigma,Z),\C)$ by
  \begin{equation*}
    \delta_{\iota}\fL^\C(n)
    \coloneq
    \int_\Sigma \iota^* i(n)\Omega
  \end{equation*} 
  for $\iota\in\Imm(\Sigma,Z)$ and $n\in T_{\iota}\Imm(\Sigma,Z)=\Gamma(\Sigma,\iota^*TZ)$.
\end{definition}

\begin{prop}
  ~
  \label{Prop_LFunctionalC}
  \begin{enumerate}
  \item
    \label{Prop_LFunctionalC_Critical}
    An immersion $\iota \colon \Sigma \to Z$ is holomorphic with respect to the conformal structure induced from $\iota^*g$ if and only if $\delta_\iota\fL^\C = 0$ and $\iota^*\omega$ is positive.
  \item
    \label{Prop_LFunctionalC_DiffInvariant}
    $\delta\fL^\C$ is $\Diff_+(\Sigma)$--invariant.
  \item
    \label{Prop_LFunctionalC_Closed}
    There is a $\Diff_+(\Sigma)$--equivariant covering space $\pi\co \tImm(\Sigma,Z) \to \Imm(\Sigma,Z)$ and a $\Diff_+(\Sigma)$--equivariant function $\tilde\fL^\C\co \tImm(\Sigma,Z) \to \C$ whose derivative is  $\pi^*\delta\fL^\C$. 
  \end{enumerate}
  
\end{prop}
\begin{proof}
  This is an analogue of \autoref{Prop_LFunctional}.
  To prove \itref{Prop_LFunctionalC_Critical} we can use the dimensional reduction of the associator identity \eqref{Eq_AssociatorIdentity}:
  \begin{equation*}
    |\omega(u,v)|^2 + |i(u,v)\Re\Omega|^2 = |u\wedge v|^2
  \end{equation*}
  for all tangent vectors $u$, $v$ to $Z$.
  The condition $\delta_\iota\fL^\C = 0$ is equivalent to $i(u,v)\Re\Omega=0$ whenever $u$ and $v$ are tangent to $\im\iota$. 
  On the other hand, by Wirtinger's inequality, the equality $\iota^*\omega = \vol_{\iota^*g}$ is equivalent to $\iota$ being holomorphic.
  The function $\tilde\fL^\C$ from \itref{Prop_LFunctionalC_Closed} is constructed by integrating $\Omega$ along $3$--dimensional chains bounding $\Sigma$.
\end{proof}

Given a complex curve $\Sigma$ one can also consider a holomorphic analogue of the Chern--Simons--Dirac functional \cite[Section 7]{Nakajima2015}.
For a triple $(A,\psi_1,\psi_2)\in \sA(\det(W))\times\Gamma(L)\times\Omega^{1,0}(\Sigma,L^*)$ define
\begin{equation*}
  \CSD^\C(A,\psi_1,\psi_2) \coloneq \int_\Sigma \delbar_A\psi_1\wedge\psi_2. 
\end{equation*}
The functional is invariant under the action of the group of complex gauge transformations $C^{\infty}(\Sigma,\C^*)$ and its critical points are triples satisfying the first two equations of  \eqref{Eq_Vortex}.
The point of \autoref{Thm_VortexCorrespondence} is that the $C^{\infty}(\Sigma,\C^*)$--equivalence classes of such triples are in one-to-one correspondence with $C^{\infty}(\Sigma,\U(1))$--equivalence classes of solutions of the full equation  \eqref{Eq_Vortex} and so the critical locus of $\CSD^\C$ consists of effective divisors on $\Sigma$.

For every coupling constant $\kappa > 0$, we can consider the coupled functional
\begin{equation*}
  \fL\CSD^\C_\kappa(\iota,A,\psi_1,\psi_2)
  =
  \fL^\C(\iota) 
  + \kappa \CSD^\C(A,\psi_1,\psi_2).
\end{equation*}
Here we use the conformal structure on $\Sigma$ induced from $\iota$ to write down the integral $\CSD^\C$.
Moreover, we identify the bundles of $(0,1)$--forms for different conformal structures, in the same way that we identified the spinor bundles of different metrics before.
The critical points of $\fL\CSD^\C_\kappa$ are solutions to a coupled system of equations similar to \eqref{Eq_IotaClassicalSeibergWitten} and \eqref{Eq_PsiAssociative}.
Solutions of the limiting equation $\kappa \to 0$ correspond to pairs consisting of a holomorphic curve and an effective divisor, as in \autoref{Sec_StablePairs}.

However, in this case the second equation of \eqref{Eq_Vortex}, obtained by varying $A$, implies that one of the sections $\psi_1$, $\psi_2$ must vanish and so the term obtained by varying $\CSD^\C(A,\psi_1,\psi_2)$ with respect to the immersion $\iota$
\begin{equation*}
 \int_\Sigma (\delta_{\iota}\delbar_A)\psi_1\wedge\psi_2
\end{equation*}
also vanishes. 
As a result, for every $\kappa$ the critical points of $ \fL\CSD^\C_\kappa$ are pairs consisting of a holomorphic curve $\Sigma$ and an effective divisor on $\Sigma$.
This suggests that there should be an enumerative theory counting such pairs in a Calabi--Yau $3$--fold.

\begin{remark}
 The fact that the critical points of $\fL\CSD^\C_\kappa$ do not depend on $\kappa$ seems to be a special feature of the Seiberg--Witten equation \eqref{Eq_Vortex}, and not a general phenomenon. 
 In particular, we do not expect it to hold for more general Seiberg--Witten equations. 
 In any case, in the limit $\kappa\to 0$ the critical point equation always decouples.
\end{remark}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "CountingAssociativesSeibergWitten"
%%% End:

